Comparison of Data Representations and Machine Learning Architectures for User Identification on Arbitrary Motion Sequences

Reliable and robust user identification and authentication are important and often necessary requirements for many digital services. It becomes paramount in social virtual reality (VR) to ensure trust, specifically in digital encounters with lifelike realistic-looking avatars as faithful replications of real persons. Recent research has shown that the movements of users in extended reality (XR) systems carry user-specific information and can thus be used to verify their identities. This article compares three different potential encodings of the motion data from head and hands (scene-relative, body-relative, and body-relative velocities), and the performances of five different machine learning architectures (random forest, multi-layer perceptron, fully recurrent neural network, long-short term memory, gated recurrent unit). We use the publicly available dataset "Talking with Hands" and publish all code to allow reproducibility and to provide baselines for future work. After hyperparameter optimization, the combination of a long-short term memory architecture and body-relative data outperformed competing combinations: the model correctly identifies any of the 34 subjects with an accuracy of 100% within 150 seconds. Altogether, our approach provides an effective foundation for behaviometric-based identification and authentication to guide researchers and practitioners. Data and code are published under https://go.uniwue.de/58w1r.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> results/2021-08-21/data_hps/accuracy_report.tex <==
\footnotesize
\begin{tabular}{llll|lll}
\toprule
 {} &   \multicolumn{3}{c}{mean accuracy} & \multicolumn{3}{|c}{minimum accuracy} \\
\midrule
{} &           SR (offset) &   BR &  BRV  &   SR (offset) &   BR &  BRV \\
\midrule
R.F.      &  77\% (17\%) &  59\% &  29\%  &   2\% (0\%) &  9\% &   0\% \\
MLP       &  91\% (6\%) &  59\% &  47\%  &  43\% (0\%) &  1\% &   7\% \\
FRNN      &  90\% (11\%) &  75\% &  59\%  &  44\% (0\%) &  9\% &  17\% \\
LSTM      &  89\% (3\%) &  59\% &  71\%  &  31\% (0\%) &  1\% &  22\% \\
GRU       &  90\% (3\%) &  61\% &  76\%  &  54\% (0\%) &  3\% &  33\% \\
\bottomrule
\end{tabular}


% \begin{tabular}{lllll}
% \toprule
% {} &   SR & SR offset &   BR &  BRV \\
% \midrule
% R. Forest &  77\% &       17\% &  59\% &  29\% \\
% MLP       &  91\% &        6\% &  59\% &  47\% \\
% FRNN      &  90\% &       11\% &  75\% &  59\% \\
% LSTM      &  89\% &        3\% &  59\% &  71\% \\
% GRU       &  90\% &        3\% &  61\% &  76\% \\
% \bottomrule
% \end{tabular}


% \begin{tabular}{lllll}
% \toprule
% {} &   SR & SR offset &  BR &  BRV \\
% \midrule
% R. Forest &   2\% &        0\% &  9\% &   0\% \\
% MLP       &  43\% &        0\% &  1\% &   7\% \\
% FRNN      &  44\% &        0\% &  9\% &  17\% \\
% LSTM      &  31\% &        0\% &  1\% &  22\% \\
% GRU       &  54\% &        0\% &  3\% &  33\% \\
% \bottomrule
% \end{tabular}





==> results/2021-08-21/data_hps/kappa_report.tex <==
\begin{table}
\centering
\caption{kappa score on test data}
\label{tab:kappa_report}
\begin{tabular}{lrrrr}
\toprule
{} &   SR & SR offset &   BR &  BRV \\
{} & test &      test & test & test \\
\midrule
R. Forest & 0.78 &      0.17 & 0.59 & 0.28 \\
MLP       & 0.91 &      0.03 & 0.60 & 0.47 \\
FRNN      & 0.91 &      0.08 & 0.75 & 0.59 \\
LSTM      & 0.91 &     -0.00 & 0.61 & 0.73 \\
GRU       & 0.92 &      0.01 & 0.61 & 0.77 \\
\bottomrule
\end{tabular}
\end{table}


==> results/2021-08-21/data_hps/min_accuracy_report.tex <==
\begin{tabular}{lllll}
\toprule
{} &   SR & SR offset &  BR &  BRV \\
\midrule
R. Forest &   2\% &        0\% &  9\% &   0\% \\
MLP       &  43\% &        0\% &  1\% &   7\% \\
FRNN      &  44\% &        0\% &  9\% &  17\% \\
LSTM      &  31\% &        0\% &  1\% &  22\% \\
GRU       &  54\% &        0\% &  3\% &  33\% \\
\bottomrule
\end{tabular}


==> results/2021-08-21/data_hps/missclassified_takes_report.tex <==
\centering
\footnotesize
\begin{tabular}{llll}
\toprule
{} & SR (offset) & BR & BRV \\
\midrule
Random Forest &  4 (25) &  2 &   4 \\
MLP       &  0 (32) &  1 &   0 \\
FRNN      &  0 (31) &  0 &   0 \\
LSTM      &  0 (34) &  7 &   0 \\
GRU       &  0 (34) &  2 &   0 \\
\bottomrule
\end{tabular}


==> results/2021-08-21/data_hps/winner_configurations.tex <==
\begin{table*}
\centering
\caption{Final configurations after architecture and data hyperparameter search; training time marks the time after which the best minimum accuracy score was achieved during training.}
\label{tab:configurations}
\begin{tabular}{llllr}
\toprule
    &     &                                                    architecture &              sample configuration &  training time \\
\midrule
RF & SR &                  n\_estimators: 85; min\_samples\_leaf: $8e+01$ &              90 frames (1 second) &           10.0 \\
    & BR &                 n\_estimators: 180; min\_samples\_leaf: $9e+02$ &              90 frames (1 second) &           10.0 \\
    & BRV &                 n\_estimators: 89; min\_samples\_leaf: $10^{1}$ &              90 frames (1 second) &           10.0 \\
MLP & SR &                 layers: 1; layer size: 204; learning rate: 0.00 &              90 frames (1 second) &           10.0 \\
    & BR &                  layers: 3; layer size: 18; learning rate: 0.01 &              90 frames (1 second) &           10.0 \\
    & BRV &                  layers: 6; layer size: 83; learning rate: 0.05 &          350 frames (3.9 seconds) &           10.0 \\
LSTM & SR &    layers: 4; layer size: 20; dropout: 0.30; learning rate: nan &      30 frames, 30 fps (1 second) &           10.0 \\
    & BR &   layers: 3; layer size: 20; dropout: 0.42; learning rate: 0.00 &      30 frames, 30 fps (1 second) &           10.0 \\
    & BRV &  layers: 3; layer size: 160; dropout: 0.01; learning rate: 0.00 &  100 frames, 90 fps (1.1 seconds) &           10.0 \\
GRU & SR &  layers: 3; layer size: 140; dropout: 0.16; learning rate: 0.00 &      30 frames, 30 fps (1 second) &           10.0 \\
    & BR &   layers: 5; layer size: 60; dropout: 0.50; learning rate: 0.01 &   100 frames, 10 fps (10 seconds) &           10.0 \\
    & BRV &  layers: 3; layer size: 160; dropout: 0.05; learning rate: 0.01 &   300 frames, 10 fps (30 seconds) &           10.0 \\
\bottomrule
\end{tabular}
\end{table*}


==> results/report/missclassified_takes_report.tex <==
\begin{tabular}{llll}
\toprule
{} & SR & BR & BRV \\
\midrule
RF   &  2 &  0 &   1 \\
FRNN &  0 &  1 &   0 \\
LSTM &  0 &  0 &   0 \\
GRU  &  0 &  0 &   0 \\
MLP  &  0 &  0 &   0 \\
\bottomrule
\end{tabular}


==> sections/tables/03_data_selection_comparison.tex <==
\begin{table*}[ht]
\caption{\label{tab:data_selections} Ten example records from the used dataset and their respective representations in the SR, BR and BRV formats.}

\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
{} & \multicolumn{6}{l}{scene-relative data} & \multicolumn{6}{l}{body-relative data} & \multicolumn{6}{l}{body-relative velocity data} \\
{} &    pos-x & pos-y & pos-z & rot-x & rot-y & rot-z &    pos-x & pos-y & pos-z & rot-x & rot-y & rot-z &    pos-x' & pos-y' & pos-z' & rot-x' & rot-y' & rot-z' \\
time &          &       &       &       &       &       &          &       &       &       &       &       &          &       &       &       &       &       \\
\midrule
0    &    -0.26 & -1.81 & 14.08 &  1.98 & -0.64 & -2.13 &    -1.79 &  0.53 & -0.55 &  1.98 & -0.64 &  2.55 &        - &     - &     - &     - &     - &     - \\
1    &    -0.27 & -1.80 & 14.08 &  1.99 & -0.64 & -2.14 &    -1.79 &  0.54 & -0.55 &  1.99 & -0.64 &  2.54 &     0.00 & -0.01 & -0.01 & -0.01 & -0.00 &  0.01 \\
2    &    -0.26 & -1.80 & 14.06 &  1.98 & -0.64 & -2.13 &    -1.79 &  0.54 & -0.55 &  1.98 & -0.64 &  2.55 &    -0.00 & -0.01 &  0.00 &  0.01 &  0.01 & -0.01 \\
3    &     3.64 &  0.26 & 15.44 &  1.77 & -0.84 & -2.58 &    -1.96 &  0.28 & -0.68 &  1.77 & -0.84 & -2.92 &     0.17 &  0.26 &  0.13 &  0.21 &  0.20 & -0.81 \\
4    &     3.73 &  0.73 & 14.81 &  1.40 & -0.29 & -2.56 &    -1.89 &  0.02 & -0.99 &  1.40 & -0.29 & -2.44 &    -0.06 &  0.26 &  0.30 &  0.37 & -0.55 & -0.48 \\
5    &     3.63 &  0.83 & 14.64 &  1.11 & -0.37 & -2.17 &    -1.85 &  0.15 & -1.10 &  1.11 & -0.37 & -2.16 &    -0.04 & -0.13 &  0.11 &  0.29 &  0.08 & -0.28 \\
6    &     3.64 &  0.52 & 15.39 &  2.28 & -0.93 & -2.71 &    -2.01 & -0.11 & -0.62 &  2.28 & -0.93 & -2.74 &     0.16 &  0.26 & -0.47 & -1.16 &  0.56 &  0.59 \\
7    &     3.78 &  0.12 & 15.41 &  1.58 & -0.44 & -2.08 &    -2.04 & -0.17 & -0.73 &  1.58 & -0.44 & -2.42 &     0.03 &  0.06 &  0.11 &  0.70 & -0.49 & -0.32 \\
8    &     3.55 &  1.12 & 12.93 &  1.53 & -0.33 & -2.67 &    -1.78 &  0.05 & -1.17 &  1.53 & -0.33 & -2.57 &    -0.26 & -0.21 &  0.44 &  0.05 & -0.11 &  0.15 \\
9    &     3.40 &  0.24 & 12.84 &  1.64 & -0.29 & -2.35 &    -1.82 & -0.06 & -1.12 &  1.64 & -0.29 & -2.59 &     0.04 &  0.11 & -0.05 & -0.12 & -0.04 &  0.01 \\
\bottomrule
\end{tabular}
}
\end{table*}

